Improving Long-Term Metrics in Recommendation Systems using Short-Horizon Reinforcement Learning

We study session-based recommendation scenarios where we want to recommend items to users during sequential interactions to improve their long-term utility. Optimizing a long-term metric is challenging because the learning signal (whether the recommendations achieved their desired goals) is delayed and confounded by other user interactions with the system. Targeting immediately measurable proxies such as clicks can lead to suboptimal recommendations due to misalignment with the long-term metric. We develop a new reinforcement learning algorithm called Short Horizon Policy Improvement (SHPI) that approximates policy-induced drift in user behavior across sessions. SHPI is a straightforward modification of episodic RL algorithms for session-based recommendation, that additionally gives an appropriate termination bonus in each session. Empirical results on four recommendation tasks show that SHPI can outperform state-of-the-art recommendation techniques like matrix factorization with offline proxy signals, bandits with myopic online proxies, and RL baselines with limited amounts of user interaction.

==> figures/fig1_data_schema.tex <==

\begin{figure}[h]
\centering
\resizebox{0.99\linewidth}{!}{
    \centering



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,1116); %set diagram left start at 0, and has height of 1116

%Shape: Circle [id:dp4879913987331652] 
\draw   (198.83,428.17) .. controls (198.83,414.36) and (210.03,403.17) .. (223.83,403.17) .. controls (237.64,403.17) and (248.83,414.36) .. (248.83,428.17) .. controls (248.83,441.97) and (237.64,453.17) .. (223.83,453.17) .. controls (210.03,453.17) and (198.83,441.97) .. (198.83,428.17) -- cycle ;
%Shape: Circle [id:dp3360463450682538] 
\draw   (91.33,519.1) .. controls (91.33,505.29) and (102.53,494.1) .. (116.33,494.1) .. controls (130.14,494.1) and (141.33,505.29) .. (141.33,519.1) .. controls (141.33,532.91) and (130.14,544.1) .. (116.33,544.1) .. controls (102.53,544.1) and (91.33,532.91) .. (91.33,519.1) -- cycle ;
%Straight Lines [id:da07802447790505584] 
\draw [line width=1.5]    (137,504.25) -- (198.29,437.94) ;
\draw [shift={(201,435)}, rotate = 492.74] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12.77,-6.13) -- (0,0) -- (12.77,6.13) -- cycle    ;
%Shape: Circle [id:dp45412604894235886] 
\draw   (91.83,429.1) .. controls (91.83,415.29) and (103.03,404.1) .. (116.83,404.1) .. controls (130.64,404.1) and (141.83,415.29) .. (141.83,429.1) .. controls (141.83,442.91) and (130.64,454.1) .. (116.83,454.1) .. controls (103.03,454.1) and (91.83,442.91) .. (91.83,429.1) -- cycle ;
%Straight Lines [id:da6531829670778508] 
\draw [line width=1.5]    (116.83,454.1) -- (116.38,490.1) ;
\draw [shift={(116.33,494.1)}, rotate = 270.72] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12.77,-6.13) -- (0,0) -- (12.77,6.13) -- cycle    ;
%Straight Lines [id:da813854695850331] 
\draw [line width=1.5]    (141.83,428.17) -- (194.83,428.17) ;
\draw [shift={(198.83,428.17)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12.77,-6.13) -- (0,0) -- (12.77,6.13) -- cycle    ;
%Shape: Circle [id:dp946566876883941] 
\draw   (198.23,357.77) .. controls (198.23,343.96) and (209.43,332.77) .. (223.23,332.77) .. controls (237.04,332.77) and (248.23,343.96) .. (248.23,357.77) .. controls (248.23,371.57) and (237.04,382.77) .. (223.23,382.77) .. controls (209.43,382.77) and (198.23,371.57) .. (198.23,357.77) -- cycle ;
%Straight Lines [id:da8896360732671211] 
\draw [line width=1.5]    (223.83,403.17) -- (223.35,386.76) ;
\draw [shift={(223.23,382.77)}, rotate = 448.32] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12.77,-6.13) -- (0,0) -- (12.77,6.13) -- cycle    ;
%Shape: Circle [id:dp9678609771215334] 
\draw   (92.23,359.77) .. controls (92.23,345.96) and (103.43,334.77) .. (117.23,334.77) .. controls (131.04,334.77) and (142.23,345.96) .. (142.23,359.77) .. controls (142.23,373.57) and (131.04,384.77) .. (117.23,384.77) .. controls (103.43,384.77) and (92.23,373.57) .. (92.23,359.77) -- cycle ;
%Straight Lines [id:da24446179580719285] 
\draw [line width=1.5]    (116.83,404.1) -- (117.15,388.77) ;
\draw [shift={(117.23,384.77)}, rotate = 451.19] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12.77,-6.13) -- (0,0) -- (12.77,6.13) -- cycle    ;
%Rounded Rect [id:dp687010783637144] 
\draw   (61.67,367.53) .. controls (61.67,343.86) and (80.86,324.67) .. (104.53,324.67) -- (233.13,324.67) .. controls (256.81,324.67) and (276,343.86) .. (276,367.53) -- (276,517.13) .. controls (276,540.81) and (256.81,560) .. (233.13,560) -- (104.53,560) .. controls (80.86,560) and (61.67,540.81) .. (61.67,517.13) -- cycle ;
%Straight Lines [id:da10122145858554332] 
\draw [line width=1.5]  [dash pattern={on 1.69pt off 2.76pt}]  (128.5,496.25) -- (202.2,379.38) ;
\draw [shift={(204.33,376)}, rotate = 482.24] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12.77,-6.13) -- (0,0) -- (12.77,6.13) -- cycle    ;
%Straight Lines [id:da0061050350301923295] 
\draw [line width=1.5]  [dash pattern={on 1.69pt off 2.76pt}]  (48.97,270.7) -- (81.67,270.7) ;
\draw [shift={(85.67,270.7)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12.77,-6.13) -- (0,0) -- (12.77,6.13) -- cycle    ;
%Straight Lines [id:da8997098205968672] 
\draw [line width=1.5]    (48.33,253.67) -- (82,253.67) ;
\draw [shift={(86,253.67)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12.77,-6.13) -- (0,0) -- (12.77,6.13) -- cycle    ;
%Straight Lines [id:da981349566217198] 
\draw [line width=1.5]  [dash pattern={on 1.69pt off 2.76pt}]  (277.3,422.03) -- (342,422.03) ;
\draw [shift={(346,422.03)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12.77,-6.13) -- (0,0) -- (12.77,6.13) -- cycle    ;
%Rounded Rect [id:dp19178212545510953] 
\draw   (39.67,360.67) .. controls (39.67,329.37) and (65.04,304) .. (96.33,304) -- (533,304) .. controls (564.3,304) and (589.67,329.37) .. (589.67,360.67) -- (589.67,530.67) .. controls (589.67,561.96) and (564.3,587.33) .. (533,587.33) -- (96.33,587.33) .. controls (65.04,587.33) and (39.67,561.96) .. (39.67,530.67) -- cycle ;
%Straight Lines [id:da8928873996856559] 
\draw [line width=1.5]    (62,429.1) -- (87.83,429.1) ;
\draw [shift={(91.83,429.1)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12.77,-6.13) -- (0,0) -- (12.77,6.13) -- cycle    ;
%Straight Lines [id:da6494789361471451] 
\draw [line width=1.5]    (223.83,453.17) -- (223.83,488.75) ;
\draw [shift={(223.83,492.75)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12.77,-6.13) -- (0,0) -- (12.77,6.13) -- cycle    ;
%Shape: Circle [id:dp9919714178622827] 
\draw   (198.83,516.6) .. controls (198.83,502.79) and (210.03,491.6) .. (223.83,491.6) .. controls (237.64,491.6) and (248.83,502.79) .. (248.83,516.6) .. controls (248.83,530.41) and (237.64,541.6) .. (223.83,541.6) .. controls (210.03,541.6) and (198.83,530.41) .. (198.83,516.6) -- cycle ;
%Straight Lines [id:da8962862851470055] 
\draw [line width=1.5]    (248.83,428.17) -- (272,428.17) ;
\draw [shift={(276,428.17)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12.77,-6.13) -- (0,0) -- (12.77,6.13) -- cycle    ;
%Shape: Circle [id:dp20731162546008108] 
\draw   (482.83,428.17) .. controls (482.83,414.36) and (494.03,403.17) .. (507.83,403.17) .. controls (521.64,403.17) and (532.83,414.36) .. (532.83,428.17) .. controls (532.83,441.97) and (521.64,453.17) .. (507.83,453.17) .. controls (494.03,453.17) and (482.83,441.97) .. (482.83,428.17) -- cycle ;
%Shape: Circle [id:dp5483791449567288] 
\draw   (375.33,519.1) .. controls (375.33,505.29) and (386.53,494.1) .. (400.33,494.1) .. controls (414.14,494.1) and (425.33,505.29) .. (425.33,519.1) .. controls (425.33,532.91) and (414.14,544.1) .. (400.33,544.1) .. controls (386.53,544.1) and (375.33,532.91) .. (375.33,519.1) -- cycle ;
%Straight Lines [id:da2314289222967798] 
\draw [line width=1.5]    (421,504.25) -- (482.29,437.94) ;
\draw [shift={(485,435)}, rotate = 492.74] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12.77,-6.13) -- (0,0) -- (12.77,6.13) -- cycle    ;
%Shape: Circle [id:dp01994129376358411] 
\draw   (375.83,429.1) .. controls (375.83,415.29) and (387.03,404.1) .. (400.83,404.1) .. controls (414.64,404.1) and (425.83,415.29) .. (425.83,429.1) .. controls (425.83,442.91) and (414.64,454.1) .. (400.83,454.1) .. controls (387.03,454.1) and (375.83,442.91) .. (375.83,429.1) -- cycle ;
%Straight Lines [id:da7650631656852094] 
\draw [line width=1.5]    (400.83,454.1) -- (400.38,490.1) ;
\draw [shift={(400.33,494.1)}, rotate = 270.72] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12.77,-6.13) -- (0,0) -- (12.77,6.13) -- cycle    ;
%Straight Lines [id:da1168364114881546] 
\draw [line width=1.5]    (425.83,428.17) -- (478.83,428.17) ;
\draw [shift={(482.83,428.17)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12.77,-6.13) -- (0,0) -- (12.77,6.13) -- cycle    ;
%Shape: Circle [id:dp7077003024031079] 
\draw   (482.23,357.77) .. controls (482.23,343.96) and (493.43,332.77) .. (507.23,332.77) .. controls (521.04,332.77) and (532.23,343.96) .. (532.23,357.77) .. controls (532.23,371.57) and (521.04,382.77) .. (507.23,382.77) .. controls (493.43,382.77) and (482.23,371.57) .. (482.23,357.77) -- cycle ;
%Straight Lines [id:da8748442489718098] 
\draw [line width=1.5]    (507.83,403.17) -- (507.35,386.76) ;
\draw [shift={(507.23,382.77)}, rotate = 448.32] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12.77,-6.13) -- (0,0) -- (12.77,6.13) -- cycle    ;
%Shape: Circle [id:dp2575127087520541] 
\draw   (376.23,359.77) .. controls (376.23,345.96) and (387.43,334.77) .. (401.23,334.77) .. controls (415.04,334.77) and (426.23,345.96) .. (426.23,359.77) .. controls (426.23,373.57) and (415.04,384.77) .. (401.23,384.77) .. controls (387.43,384.77) and (376.23,373.57) .. (376.23,359.77) -- cycle ;
%Straight Lines [id:da002158834869338433] 
\draw [line width=1.5]    (400.83,404.1) -- (401.15,388.77) ;
\draw [shift={(401.23,384.77)}, rotate = 451.19] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12.77,-6.13) -- (0,0) -- (12.77,6.13) -- cycle    ;
%Rounded Rect [id:dp7078438942921834] 
\draw   (345.67,367.53) .. controls (345.67,343.86) and (364.86,324.67) .. (388.53,324.67) -- (517.13,324.67) .. controls (540.81,324.67) and (560,343.86) .. (560,367.53) -- (560,517.13) .. controls (560,540.81) and (540.81,560) .. (517.13,560) -- (388.53,560) .. controls (364.86,560) and (345.67,540.81) .. (345.67,517.13) -- cycle ;
%Straight Lines [id:da4517310588212642] 
\draw [line width=1.5]  [dash pattern={on 1.69pt off 2.76pt}]  (412.5,496.25) -- (486.2,379.38) ;
\draw [shift={(488.33,376)}, rotate = 482.24] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12.77,-6.13) -- (0,0) -- (12.77,6.13) -- cycle    ;
%Straight Lines [id:da8622032525761156] 
\draw [line width=1.5]    (346,429.1) -- (371.83,429.1) ;
\draw [shift={(375.83,429.1)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12.77,-6.13) -- (0,0) -- (12.77,6.13) -- cycle    ;
%Straight Lines [id:da40934536226168583] 
\draw [line width=1.5]    (507.83,453.17) -- (507.83,488.75) ;
\draw [shift={(507.83,492.75)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12.77,-6.13) -- (0,0) -- (12.77,6.13) -- cycle    ;
%Shape: Circle [id:dp5076680432636347] 
\draw   (482.83,516.6) .. controls (482.83,502.79) and (494.03,491.6) .. (507.83,491.6) .. controls (521.64,491.6) and (532.83,502.79) .. (532.83,516.6) .. controls (532.83,530.41) and (521.64,541.6) .. (507.83,541.6) .. controls (494.03,541.6) and (482.83,530.41) .. (482.83,516.6) -- cycle ;
%Straight Lines [id:da6451912280597849] 
\draw [line width=1.5]    (532.83,428.17) -- (556,428.17) ;
\draw [shift={(560,428.17)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12.77,-6.13) -- (0,0) -- (12.77,6.13) -- cycle    ;

% Text Node
\draw (206.83,418.67) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle X_{t+1}$};
% Text Node
\draw (107.83,510.1) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle A_{t}$};
% Text Node
\draw (108.33,421.1) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle X_{t}$};
% Text Node
\draw (208.4,349.27) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle Y_{t+1}$};
% Text Node
\draw (109.4,350.27) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle Y_{t}$};
% Text Node
\draw (243.33,529.17) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \rho $};
% Text Node
\draw (111.73,261.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle Implicit\ ( weak) \ dependence\ ( marginalized\ out)$};
% Text Node
\draw (113.73,238.93) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle Explicit\ ( strong) \ dependence\ ( conditionned)$};
% Text Node
\draw (531,562) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle N$};
% Text Node
\draw (207.33,507.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle A_{t+1}$};
% Text Node
\draw (490.83,418.67) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle X_{t+1}$};
% Text Node
\draw (391.83,510.1) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle A_{t}$};
% Text Node
\draw (392.33,421.1) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle X_{t}$};
% Text Node
\draw (492.4,349.27) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle Y_{t+1}$};
% Text Node
\draw (393.4,350.27) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle Y_{t}$};
% Text Node
\draw (527.33,529.17) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \rho $};
% Text Node
\draw (491.33,507.6) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle A_{t+1}$};


\end{tikzpicture}

}
\caption{Causal pattern assumed for our problem. Plate notation abstracts the notion of episode. Implicit dependence links (dotted arrows) are assumed to be \emph{weak} enough so that they can be treated as nonexistent.}
    \label{fig:causal_pattern}
\end{figure}

==> figures/fig2_problem_structure.tex <==
\begin{figure}[h!]
\centering
\resizebox{0.99\linewidth}{!}{
    \centering

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,852); %set diagram left start at 0, and has height of 852

%Rounded Rect [id:dp08260082448081585] 
\draw   (154,246.2) .. controls (154,220.5) and (174.83,199.67) .. (200.53,199.67) -- (514.63,199.67) .. controls (540.33,199.67) and (561.17,220.5) .. (561.17,246.2) -- (561.17,385.8) .. controls (561.17,411.5) and (540.33,432.33) .. (514.63,432.33) -- (200.53,432.33) .. controls (174.83,432.33) and (154,411.5) .. (154,385.8) -- cycle ;
%Rounded Rect [id:dp6047443786728182] 
\draw  [fill={rgb, 255:red, 157; green, 216; blue, 112 }  ,fill opacity=1 ] (201.83,245) .. controls (201.83,225.12) and (217.95,209) .. (237.83,209) -- (480.83,209) .. controls (500.72,209) and (516.83,225.12) .. (516.83,245) -- (516.83,353) .. controls (516.83,372.88) and (500.72,389) .. (480.83,389) -- (237.83,389) .. controls (217.95,389) and (201.83,372.88) .. (201.83,353) -- cycle ;
%Rounded Rect [id:dp7536769814719562] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (253.67,241.53) .. controls (253.67,228.35) and (264.35,217.67) .. (277.53,217.67) -- (438.63,217.67) .. controls (451.81,217.67) and (462.5,228.35) .. (462.5,241.53) -- (462.5,313.13) .. controls (462.5,326.31) and (451.81,337) .. (438.63,337) -- (277.53,337) .. controls (264.35,337) and (253.67,326.31) .. (253.67,313.13) -- cycle ;

% Text Node
\draw (258.67,298.67) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {Space solvable by stationary CB};
% Text Node
\draw (227,345.33) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {Space solvable by repeated application of\\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ stationary CB\textbf{ }(\textit{CB++}) };
% Text Node
\draw (279.67,398.67) node [anchor=north west][inner sep=0.75pt]   [align=left] {General MDP space};


\end{tikzpicture}


}
\caption{Schematic view of the class of problems studied in this work. The class of MDPs solvable by our algorithm is nested in between general MDPs and contextual bandits.}
    \label{fig:problem_class_nested}
\end{figure}

==> implementation.tex <==
\section{Implementation Details}
\label{sec:implementation}

The computational and storage costs of~\method~scale linearly with $k$, since the quantity $\hat{\mathbb{A}}^\pi_{(k)}$ can be computed in a single pass through the data. 
\method~also requires the pre-computation, or access to a scoring function $\hat{V}^\mu$ over user contexts under the behavior policy. %We restrict ourselves to the case when this role is played by the empirical estimate of the value function $\hat{V}^\mu$; it can be pre-computed efficiently using an iterative policy evaluation scheme.

% \subsection{Choice of reward estimator [DELETE?]}
% \label{sec:reward_models}
% In the $k$-step advantages of Equation~\ref{eq:advantage_MC}, we typically use Monte Carlo samples $r(X_{i,t+m},A_{i,t+m})$ to estimate the instantaneous state-action reward. However these rewards may be sparse -- for instance, product purchases may be a very small fraction of user interactions. When we have access to a value function $Y_t \equiv \hat{V}^\mu(x_t)$ as in Equation~\ref{eq:v_dm_obj}, we can replace the $\hat{r}$ estimate by recognizing that $r \approx \hat{V}^\mu(x_t) - \gamma \hat{V}^\mu(x_{t+1})$. We recommend using $\hat{r}_t=Y_{t}-Y_{t-1}=(1-\mat{B})Y_t$, where $\hat{r}_0=Y_0$ and $\mat{B}$ denotes the \emph{backshift operator}.
% The backshift reward estimator has two additional redeeming properties: (i) it isolates the effect of action $a_t$ on $x_t$ using a dense shaping reward %which makes the estimator look like 
% $\hat{r}_t=\hat{r}(X_t,A_t)$, %instead of $\hat{r}_t=\hat{r}(X_t)$, 
% and (ii) it eliminates stationary additive bias in the learned value functions or additive exogenous reward noise in the environment, if any. 





==> outline.tex <==
\subsection{Outline}
Online metrics gauge user satisfaction with recommendation systems.
Contextual bandit framing is used to optimize online metrics like clicks and other immediate user feedbacks. (\textbf{what about other methods like MF} \textit{They do not optimize online metrics, but instead they optimize some other offline proxies}). \textit{Also: MF is a model type, contextual bandit is a setting type; one could use MF with CB.  I suppose traditional MF corresponds to the direct method (i.e., ignoring coverage issues and hoping for asymptotic convergence).}  

However, we care about long-term metrics, say monthly active usage. $LTE = \frac{Clicks}{Month} = \frac{Click}{Impression}\frac{Impressions}{Session}\frac{Sessions}{Month}$.
Clicks and other immediate user feedback are too myopic for maximizing LTE, because they greedily optimize the first term even if that lowers the other two terms (eg drive-off impressions for users with very low CTR, keep those with high CTR). \textbf{(is the class of problems for which myopic metric optimization fails and LTE succeeds meaningful for practitioners?)}.\textit{Great question. That is the premise of the paper (and the example in Sec3). Need to add a paragraph for this before motivating session-based RL.} \textit{Also: succeeds/fails is a binary concept; better to show improvement over myopic optimization of large enough magnitude to be interesting.} \textbf{Also optimizing clicks/impression maximizes clicks, lowers impression, and nothing counters this minimization (is this what you mean?)} \textit{Yes.}

Session-based recommendation uses RL to reliably optimize $\frac{Clicks}{Session} = \frac{Click}{Impression}\frac{Impressions}{Session}$.
But, both click-maximizing bandits and session-based RL are ignoring that  $\frac{Sessions}{Month}$ can also depend on the deployed recommendation policy. [See Section~\ref{sec:example} for a motivating example]. \textbf{Trying to map this back to a mental image of RL, clicks=reward r(s,a) and sessions=episode, while month=long-term metric horizon? The impression is then the proxy reward as I understand?}\textit{There is no proxy reward. Episode = month. Sessions is a new concept akin to false horizon, explained in Section 2.} \textit{Also: generalizes returning is believing to false horizon value estimation.}

Our Idea. Approximate the effect of policy on $\frac{Sessions}{Month}$ by using $Sessions(policy) = \sum_{\mathrm{UserContext C}} \Pr(C \mid policy) SessionRate(C)$.
We can then estimate $\Pr(C \mid policy)$ and $SessionRate(C)$ separately using off-policy data collected from an existing recommender  system.
\textbf{Bogdan: I think when we write this in final form, it would be helpful to denote the previous as iterated expectation, e.g. $\mathbb{E}_\pi[Sessions]=\mathbb{E}_{\pi}[\mathbb{E}_{C|\pi}[SessionRate(C;\pi)]]$, which makes the conditioning explicit (at least for me). }

So we devise a practical session-based RL algorithm that can \textit{(more)} reliably optimize LTE. It is a straightforward modification of existing episodic session-based recommenders, by additionally giving an appropriate episodic termination bonus (capturing $SessionRate(C)$ for user contexts induced by the policy) in each session. \textbf{Quality of session-rate depends on the data/policy as in HuRL? }\textit{In kind of the same way, yes. Suppose $SessionRate$ actually depends on policy too. In that case, our estimate is $SessionRate=SessionRate(C, \mu)$ but what we want is $SessionRate(C, \pi^*)$. And that gap is kind of like the gap that HuRL uses to quantify the quality of a heuristic.}

Our analysis shows that the algorithm interpolates between two traditional policy improvement schemes, and inherits reliable policy improvement guarantees. 
Adapting recent results in short-horizon RL~\cite{HuRL} to the off-policy setting, we can also relate approximation quality of $SessionRate(C)$
to the quality of LTE optimization.

Our experiments show that our algorithm is simple to run, can be adapted to work with off-policy data, and outperforms session-based, contextual bandit and other recommendation baselines on a wide variety of LTE objectives. 

WHAT WILL NOT BE DISCUSSED:
\begin{itemize}
    \item Proxy LTE predictor. Using backshift to derive immediate rewards. 
    \item Batch RL concepts like  pessimism, trust region etc.
    \item Other solution strategies like model-based RL, CPI, PPO.
    \item Changing the ``false horizon'' $k$? \textit{If I had to choose one thing to keep in this list, it's this one.  Unless it doesn't matter with a long-enough horizon and truncated importance weights (?).  We should at least demonstrate a lack of sensitivity.}
\end{itemize}
